K-QA: A Real-World Medical Q&A Benchmark

Ensuring the accuracy of responses provided by large language models (LLMs) is crucial, particularly in clinical settings where incorrect information may directly impact patient health. To address this challenge, we construct K-QA, a dataset containing 1,212 patient questions originating from real-world conversations held on K Health (an AI-driven clinical platform). We employ a panel of in-house physicians to answer and manually decompose a subset of K-QA into self-contained statements. Additionally, we formulate two NLI-based evaluation metrics approximating recall and precision: (1) comprehensiveness, measuring the percentage of essential clinical information in the generated answer and (2) hallucination rate, measuring the number of statements from the physician-curated response contradicted by the LLM answer. Finally, we use K-QA along with these metrics to evaluate several state-of-the-art models, as well as the effect of in-context learning and medically-oriented augmented retrieval schemes developed by the authors. Our findings indicate that in-context learning improves the comprehensiveness of the models, and augmented retrieval is effective in reducing hallucinations. We make K-QA available to to the community to spur research into medically accurate NLP applications.

==> sections/01_introduction.tex <==
Large Language Models (LLMs) have garnered significant attention due to their impressive capabilities in generating natural language \citep{wei2022emergent}. However, their reliance on pre-training to model statistical correlations between tokens renders them susceptible to generating text that lacks factual accuracy \citep{ji2023survey, bang2023multitask}.
% , commonly referred to as \textit{hallucinations} 
Ensuring trustworthy text from question answering (QA) systems is crucial in real-world applications, particularly in the medical domain \citep{shen2023chatgpt}. The accuracy of responses to consumer health questions, frequently asked by the general public, is imperative given the potential significant consequences and the public's limited capacity to evaluate the quality of medical content \citep{jin2022biomedical}.
% Providing accurate answers to consumer health questions, commonly posed by the general public, is essential due to potential impactful consequences and the public's limited ability to assess the quality of medical content \citep{jin2022biomedical}.

Recognizing this, we introduce \kqa{}, a long-form question answering benchmark derived from authentic patient-physician interactions, capturing the nuanced nature of medical discourse. 
Our dataset has undergone rigorous curation by medical professionals, upholding the highest standards of accuracy, validity, and responsibility. Physicians provide thoughtful responses to each question, incorporating relevant medical considerations, even if not directly answering the question. 
For instance, in response to the question \emph{"What's good for muscular pain?"}, the reply contains a red-flag statement such as \emph{"Seek medical attention if you have numbness or tingling in limbs"}, providing necessary information beyond the patient's inquiry.
% For example, in response to the question \emph{What's good for muscular pain?}, the reply contains a red-flag statement such as \emph{Seek medical attention if you have numbness or tingling in limbs}, providing necessary information beyond the patient's inquiry.
% Our dataset underwent rigorous curation by medical professionals, upholding the highest standards of accuracy, validity, and responsibility. This is demonstrated through thorough medical considerations, which may also include responses that are not always direct answers to patients' questions (e.g., \emph{"seek medical attention if you have neck muscle stiffness while swallowing"}).
% \ran{consider adding the question. I'm not sure it's clear only with the answer}
\kqa{} consists of questions from patients and responses from physicians, presenting both free-form and granular-form self-contained statements. These statements are categorized according to their clinical significance, as illustrated in Figure \ref{fig:example}.

% The physicians' curated responses are available in both free-form and decomposed formats into statements, categorized according to their clinical importance (as depicted in Figure \ref{fig:example}).
% Ensuring trustworthy and reliable text from LLMs is crucial in real-world applications, particularly in the medical domain \citep{shen2023chatgpt}. With a focus on consumer health questions, which are commonly posed by the general public, delivering accurate answers is critically vital due to their potentially impactful consequences and the public's limited ability to assess the quality of medical content \citep{jin2022biomedical}. 
% Producing trustworthy and accurate text is paramount when using LLMs in real-world applications, especially in the medical domain, where reliability is essential \citep{shen2023chatgpt}. With a focus on consumer health questions, which are commonly posed by the general public, delivering accurate answers is critically vital due to their potentially impactful consequences and the public's limited ability to assess the quality of medical content \citep{jin2022biomedical}.\itay{add something about the importance of a model to answer "I don't know"}
% In light of this, we introduce \kqa{}, a unique benchmark sourced from real patient-physician interactions, capturing the intricate nuances of medical discourse. Notably, our dataset stands out for its rigorous curation, involving thorough scrutiny and revision by a panel of expert medical professionals. This meticulous process guarantees that our dataset not only mirrors real medical inquiries but also upholds the highest standards of accuracy and validity.
% \ran{maybe also stating that this dataset also includes a very high standard of responsibility, manifested in statements that are not always a direct answer to the question (e.g. if you feel x you should seek immediate medical attention)}
% \itay{Here - write about decomposition of statements}

% Ensuring trustworthy and reliable text from LLMs is crucial in real-world applications, particularly in the medical domain \citep{shen2023chatgpt}. With a focus on consumer health questions, which are commonly posed by the general public, delivering accurate answers is critically vital due to their potentially impactful consequences and the public's limited ability to assess the quality of medical content \citep{jin2022biomedical}

\itay{A paragraph on the need of standard automatic evaluation metric
Human evaluation continues to serve as the reference standard for appraising the faithfulness of text produced by automated systems, even though its application involves substantial costs, limitations in scalability, intricate replicability, and the time-consuming aspect attributed to the frequently extended length of the generated text \citep{krishna2023longeval, gehrmann2023repairing}. 
Since there currently exists no “perfect” metric, we will not conclude with explicit metric recommendations but rather try and extract successful metric design principles alongside a family of evaluations that together may provide a more complete characterization of a model’s performance.}

We propose two innovative metrics inspired by recent work on fine-grained factuality \citep{chen2022propsegment, min2023factscore}: \emph{Comprehensiveness}, measuring the presence of clinically important statements, and \emph{Hallucination rate}, 
\ran{I feel more comfortable with ``inaccuracies'' or ``mistakes'' because it's mostly not terrible errors. Your call.} quantifying the extent of contradictions in a generated response compared to physicians' statements.
% quantifying contradictions with physicians' statements. 
Our interpretation of hallucinations diverges from traditional definitions, which commonly denote claims without external grounding \citep{ji2023survey}. 
Instead, we specifically identify hallucinations as contradictions to physician statements, which we believe pose greater risks.
A reliable system should cover all essential clinical components and align with physicians, demonstrating high \emph{comprehensiveness} and an absence of \emph{hallucination}.
% We propose two novel metrics inspired by recent work on fine-grained factuality \citep{chen2022propsegment, min2023factscore}: \emph{Comprehensiveness}, which measures the presence of clinically important statements, and \emph{Hallucination rate}, which quantifies the extent of contradictions in a generated response compared to the physicians' statements. Unlike common definitions of hallucinations, typically referring to claims not grounded in external sources \citep{ji2023survey}, we define hallucinations as contradictions to physician statements, which we believe pose greater risks.
% A reliable system should cover all essential clinical components and align with physicians, demonstrating high \emph{comprehensiveness} and an absence of \emph{hallucination}.

Our empirical study across several state-of-the-art models reveals the challenging nature of the \kqa{} benchmark. The highest comprehensiveness score is below 68\%, indicating that the models struggle to incorporate statements deemed important by physicians. Additionally, all of the models exhibited hallucinations. The optimal balance was found with Retrieval Augmented Generation (RAG; \citealp{lewis2020retrieval}) and an engineered prompt for GPT-3.5, resulting in the lowest \emph{hallucination rate}.


The contributions of our work can be summarized as follows:
\begin{itemize}[left=0em, itemsep=-1ex]
%, before=\vspace{-\baselineskip}]
\item We created a new, free-form high-quality dataset for medical question-answering, derived from a diverse range of real-world patients' questions accompanied by meticulously curated physician answers.
\item We introduced two novel evaluation metrics for factuality, enabling granular scoring of generated text, considering statements and weights.
\item We evaluated the performance of state-of-the-art models, including GPT-3.5, GPT-4, Mistral, PALM-2, and commercial generative services BARD and Bing, on the \kqa{} benchmark.
\end{itemize}

% The contributions of our work can be summarized as follows:
% \begin{itemize}[left=0em, itemsep=-1ex, after=\vspace{-\baselineskip}]
%     \item Create a new high-quality dataset for medical question-answering, based on diverse real-world patients' questions accompanied with highly-curated physician answers. 
%     \item Novel evaluation method to estimate Precision and Recall of factuality, on atomic-level, including explainability.
%     \item We evaluate the performance of state-of-the-art models, including GPT-3.5, GPT-4, Mistral, PALM-2, and commercial generative services BARD and Bing, on the \kqa{} benchmark.
%     % \item We devise a retrieve-and-prompt technique which we show is more factually correct than state-of-the-art LLMs, both in human evaluation, as well using our new evaluation.
% \end{itemize}

% We regard \emph{hallucination} as a response contradicting physicians, considering it an error that a trustworthy system should avoid; yet, all models exhibited hallucinations. 
% The optimal balance of metrics was found with the Retrieval Augmented Generation (RAG) \citep{lewis2020retrieval} setup and an engineered prompt for GPT-3.5, resulting in the lowest \emph{hallucination rate}.
% Our empirical study across 13 state-of-the-art (SoTA) systems (including GPT-4) shows that CROW is a challenging commonsense reasoning testbed, with the highest performing model scoring ∼18% lower than humans on individual examples and ∼37% lower on our more restrictive metric that evaluates situational robustness. Consequently, we provide CROW to the community as the first com- monsense benchmark specifically formed to test commonsense knowledge and reasoning abilities in the same contexts as real-world deployments of NLP systems. The contributions of our work can be summarized as follows:
% \itay{
% IMPORTANT POINTS:
% \begin{enumerate}
%     % \item Unique Dataset: questions from Real human-physician interaction.
%     % \item Highly validated by medical experts.
%     % \item Detailed Answers which are also prioritized, and decomposed to atomic claims.
%     \item A novel generic evaluation method. An end-to-end automatic evaluation for estimating generated answers, as good as humans.
%     % \item Scoring of the evaluation can be adapt according to the task.
%     % \item Due to the latest technological advances, we are able to integrate long texts to understand intricate logical relationships based on NLI (it could not have been possible 1-2 years ago).
%     % \item benchmark to LLMs. 
% \end{enumerate}}

% \nadav{A good reference quote from Google's publication in nature: "Our human evaluations reveal limitations of today’s models, reinforcing the importance of both evaluation frameworks and method development in creating safe, helpful LLMs for clinical applications." taken from:
% https://www.nature.com/articles/s41586-023-06291-2}
% \gabi{unusual to put a subsection under the Introduction. Instead merge with the previous section.}
% \gabis{The introduction should include all major aspects of the paper. and be around a 1-1.5 pages. We can also think about a high-level Figure 1 which can give an overall picture of what we did.} \\
% \nadav{
%     \begin{itemize}
%       \item we can highlight here that although the contributions of this work are focused on the medical domain (medical question answering in a clinical workflow), the same techniques (besides the dataset itself) can be used for LLMs that aren't in a medical field (it's already pretty much written above, but maybe worth emphasizing)
%     \end{itemize}
% }


==> sections/04_1_task_formulation.tex <==
The objective of the \kqa{} benchmark is to evaluate the performance of free-form generative question-answering. In this task, a model can abstain from answering a question if it is expected to produce an inaccurate answer to a given query. Evaluation criteria involve ensuring the inclusion of essential elements in the response (\mh{}) and avoiding contradictions with physicians' statements, i.e., (\mh{} and \nth{}).
 \gabis{also explain that the model can abstain, and the clinical significance of \mh{} and \nth{}}\itay{I added it, but in fact I think that it should be in the evaluation and not on the task formulation}

==> sections/04_evaluation.tex <==
The objective of the evaluation is to assign a score to the model's output that accurately reflects its alignment with the factual information provided in the grounding, which in this case, is the physician's answer.
Subsequently, we proceed to provide a formal description of our approach, which hinges upon two key ideas:
\subsubsection*{Key idea 1: Weighted Atomic Claims}  
% Our approach draws inspiration from the Pyramid paradigm, introducing Semantic Content Units (SCUs) \citep{nenkova2007pyramid}, and the more recent concept of Atomic Content Units (ACUs) \citep{liu2022revisiting}. These units aim to encapsulate  concise, self-contained claims with maximum clarity. While SCUs involve weighted semantic content units for multi-reference evaluation, ACUs offer a framework without weighting. Our methodology suggests that weighting can be customized based on the chosen evaluation metric \yaara{See section \ref{definition}.
% Additionally, we provide standardized annotation guidelines, particularly for medical contexts. These guidelines cover handling complex logical relationships (e.g., XOR, AND, IF statements) and lists of medical entities (e.g., symptoms, vaccines) \itay{[see more details in the appendix]}. Although some annotator subjectivity may persist in crafting atomic claims, it won't introduce bias in the comparative evaluation, as all candidate answers are assessed using the same set of claims.
% \yaara{Shouldn't SCUs and ACUs be explained in the related work section? and what's a Pyramid paradigm?}\itay{well, i am not sure.. but we might write it differently at the end. Regarding the Pyramid - I think that I will write in one sentence, that it suggests a weighting framework, based on different candidates and annotators...} 
Our approach draws inspiration from the Pyramid paradigm, which introduced Semantic Content Units (SCUs) \citep{nenkova2007pyramid}, and the more recent concept of Atomic Content Units (ACUs) \citep{liu2022revisiting}. These units are designed to encapsulate concise, self-contained claims with maximum clarity. While ACUs provide a framework without incorporating weighting, SCUs were originally designed for multi-reference evaluation, involving the assignment of weights to semantic content units. 
Our methodology suggests that weighting can be customized based on the chosen evaluation metric \yaara{See section \ref{definition} for details on the weighting of the claims.}
Additionally, we provide standardized annotation guidelines, particularly for medical contexts. These guidelines cover handling complex logical relationships (e.g., XOR, AND, IF statements) and lists of medical entities (e.g., symptoms, vaccines) \itay{[see more details in the appendix]}.
% Additionally, we establish guidelines to standardize the annotation process, with a focus on medical contexts. We provide instructions for handling complex logical relationships, such as XOR, AND, IF statements, and lists of medical entities (e.g., symptoms, vaccines) 
 It's worth noting that some inherent subjectivity may persist among annotators when crafting atomic claims, even with the provided guidelines. Nevertheless, this subjectivity should not introduce bias in the comparative evaluation, as all candidate answers are assessed using the same set of claims.
\subsubsection*{Key idea 2: NLI-based with Chain-of-Thoughts}
In accordance with  \citep{schuster2022stretching}, we leverage LLMs to expand conventional NLI models to include paragraph-sentence pairs. Additionally, we incorporate Chain-of-Thoughts (CoT) \citep{wei2022chain}, a method that provides sequential intermediary representations generated by the LLM during text generation. 
Remarkably, through the presentation of task-specific logical reasoning examples, the language model demonstrates the capacity to autonomously generate these intricate evaluation trajectories. 
CoT plays a pivotal role in enhancing contextual understanding and providing strategic guidance for the language model's evaluation of generated text. It also helps elucidate the rationale behind the evaluation process and its results.
% The Chain-of-Thoughts (CoT) \citep{wei2022chain} embodies sequential intermediary representations that are generated by the LLM during the process of the text generation. Within the domain of evaluation tasks, specific criteria demand an extensive evaluation framework that extends beyond mere strict definitions. Remarkably, through the presentation of task-specific logical reasoning examples, the language model demonstrates the capacity to autonomously generate these intricate evaluation trajectories. The CoT serves as a means to augment contextual insight and strategic guidance for the language model's evaluation of the generated text, while simultaneously also explaining the rationale behind the evaluation procedure and its outcomes.
\yaara{This section is not clear. what model is being used here? we should probably rephrase and also add a figure with an example of evaluating one answer (we can use the Q and claims from figure \ref{fig:example})}

\subsection{Definition} \label{definition}
Let $\mathcal{M}$ be a language model, and $\mathcal{X}$ be a set of prompts, such that a response is defined as $\mathcal{M}_x$ for $x \in \mathcal{X}$. Consider $a\in\mathcal{A}_{x}$ as a claim within the set of atomic claims associated with a given question.
This evaluation is conducted within the framework of NLI, with the goal of classifying each pair of \textit{(premise, hypothesis)} into one of three categories: $\{entail, contradict, neutral\}$. Within this framework, we regard the hypothesis as the claim ($a$), and the generated response ($\mathcal{M}_x$) as the premise.

\subsection{Metrics} \label{eq:PRRE}
In our specific context, we separated $\mathcal{A}_{x}$ into two exclusive sets of claims, denotes $\mathcal{A}_{x}^{mh}$ as a \mh and $\mathcal{A}_{x}^{nh}$ as a \nth.
The \textit{Truthfulness}, which can be regarded as a measure of factual accuracy, serving as a proxy for Precision ($PR$), and the \textit{Comprehensiveness}, acting as a proxy for Recall ($RE$), at the question level, are defined as follows:
\begin{align}
    &\text{(1)} \quad PR_{x} = \frac{1}{|\mathcal{A}_{x}|}\sum_{a\in \mathcal{A}_{x}}[\mathcal{M}_{x}\text{ does not contradict }a] \notag \\
    &\text{(2)} \quad RE_{x} = \frac{1}{|\mathcal{A}_{x}^{mh}|}\sum_{a\in \mathcal{A}_{x}^{mh}}[\mathcal{M}_{x}\text{ entails }a] \notag
\end{align}
Thus, for questions that the language model did not produce responses, $RE_{x}$ will be $0$, and $PR_{x}$ will be $1$. For an explanation of how we derive these metrics from a general scoring framework please refer to the supplementary materials (Appendix \ref{app:math}). The aggregated metrics for the entire dataset are defined as follows:
\begin{align*}
    PR &= \frac{1}{|\mathcal{X}|}\sum_{x\in \mathcal{X}}PR_{x} \ \  & 
    RE = \frac{1}{|\mathcal{X}|}\sum_{x\in \mathcal{X}}RE_{x}
\end{align*}
Additionally, we introduce an aggregated metric named  $\text{contra}_{\text{norm}}$, which calculates the number of contradictions normalized per 100 questions.
\begin{align*}
\text{contra}_{\text{norm}} &= \frac{100}{n}\sum_{x\in\mathcal{X}}\sum_{a\in\mathcal{A}_{x}} [\mathcal{M}_{x}\text{ contradicts }a]
\end{align*}
In this expression, $n$ represents the total number of questions answered by the language model.

% \subsection{Definition} \label{definition}
% Let $\mathcal{M}$ be a language model, and $\mathcal{X}$ be a set of prompts, such that a response is defined as $y = \mathcal{M}_x$ for $x \in \mathcal{X}$ \itay{should i continue with $\mathcal{M}_x$ without y?}. Let $\mathcal{A}$ \itay{or $\mathcal{A}_{x}$?} denote a set of atomic claims for a given question, and let $\mathcal{W}$ \itay{$\mathcal{W}_x$?} denote the weights assigned to these atomic claims.
% Consider an NLI model, denoted as $\mathcal{N}(premise, hypothesis)$, designed to classify each pair of \textit{(premise, hypothesis)} into one of three labels: $l \in \{entail, contradict, neutral\}$. Within this framework, we view the hypothesis as the claim ($a$) \itay{DEFINE $a$} and the generated response ($y$) as the premise, denoted as $\mathcal{N}(y, a)$. We define $f(\mathcal{N}(y, a), l)$ as a function that takes the output of the NLI model and a predefined logical relation, such as "does not contradict," and returns a boolean value.
% The formula representing this process is as follows:
% \begin{align}\label{eq:1}
% \frac{\sum_{a \in \mathcal{A}} w(a) \cdot f(\mathcal{N}(y, a), l)}{\sum_{a \in \mathcal{A}} w(a)}
% \end{align}
% \itay{Or writing as follows:}
% \begin{align*}
% \frac{\sum_{i=1}^{|\mathcal{A}|} w_i \cdot f(\mathcal{N}(y, a_i), l)}{\sum_{i=1}^{|\mathcal{A}|} w_i}
% \end{align*}
% This mathematical expression quantifies how well the generated response aligns with a predefined logical condition, while taking into account the weights assigned to individual claims.  It is important to note that this definition assumes that each atomic claim in $\mathcal{A}$ is treated independently.
% \yaara{So many questions... what is the name of the weighted average listed above? how is it used? what is $w$ in our case? And if it's always 1 for precision and 1 or 0 for recall as in the next section, why do we need it? it adds complexity. I suggest showing only the Pr/Re metrics that are in the next section, and only then explain that we can generalize it with weights (and go into the details in an appendix)} 
% \itay{ok, so here we have different ways to display this metric. It is quite simple, but it gets complicated by adding more notations. I want to show that it is quite generic metric and it can be adjust by the users' desires, by only changing the weights.. and then give an example of how we were weighting the claims. I don't think that I need to have 4 equations, I just wonder if one generic is good or two specific and than trying to draw a line to the general case.}

% \subsection{Metrics} 
% In our specific context, we separated $\mathcal{A}$ into two exclusive sets of claims, denotes $\mathcal{A}_{mh}$ \itay{or $\mathcal{A}_{x}^{mh}$?} as a \mh and $\mathcal{A}_{nh}$ as a \nth.
% The \textit{Truthfulness}, which can be regarded as a measure of factual accuracy, serving as a proxy for Precision ($Pr$), and the \textit{Comprehensiveness}, acting as a proxy for Recall ($Re$), at the question level, are defined as follows:
% \begin{align}
%     Pr &= \frac{1}{|\mathcal{A}|}\sum_{a\in \mathcal{A}}[a\text{ does not contradict }y] \\
%     Re &= \frac{1}{|\mathcal{A}_{mh}|}\sum_{a\in \mathcal{A}_{mh}}[a\text{ entails }y]
% \end{align}
% \itay{Another options
% \begin{align}
%     Pr_x &= \frac{1}{|\mathcal{A}_x|}\sum_{a\in \mathcal{A}_x}[a\text{ does not contradict }\mathcal{M}_x] \\
%     Re_x &= \frac{1}{|\mathcal{A}_{x}^{mh}|}\sum_{a\in \mathcal{A}_{x}^{mh}}[a\text{ entails }\mathcal{M}_x]
% \end{align}
% }
% These metrics are aligned with the formulation of equation \ref{eq:1}. For Precision computation, $w_i$ is set to 1, whereas for Recall, $w_i$ takes the value of 1 if $a$ is in $\mathcal{A}_{mh}$ and 0 if $a$ falls within $\mathcal{A}_{nh}$.

% \itay{These metrics are calculated at the question-level. However, an aggregated metric, such as \textit{normalized contradictions}, can also be derived:
% \begin{align*}
% \frac{100}{n}\sum_{i=1}^{n}\sum_{a\in{\mathcal{A}}} [a\text{ contradicts } y_i]
% \end{align*}
% In this expression, $i$ iterates over each question-answer pair, and $n$ represents the total number of answered questions. \\
% MAYBE $\mathcal{A}_x$ is clearer.\\
% In addition, we can write the aggregated \textit{Truthfulness} as:
% \begin{align}
%     \text{Pr} = \mathbb{E}_{x\in\mathcal{X}}[Pr_x|\mathcal{M}_x \text{ responds}]
% \end{align}
% }


\subsection{Additional Metrics}
Due to the generic nature of the proposed evaluation framework, it can be easily adapted to other metrics for text generation by adjusting the weights. 
To provide an example, in the context of measuring \textit{Harmfulness}, we can create a metric that assigns higher weights to claims that emphasize medical 'red flags', such as \itay{Naama? ""}, allowing us to evaluate the safety of the generated responses.
\itay{
    \begin{enumerate}
        \item OPTIONAL: after extracting the claims that are not covered, we return them as an output for the user. This can be used for further analysis, such as \citep{kryscinski2019evaluating} \\
        "We address the problem of verifying factual consistency between source documents and generated summaries: a factually consistent summary contains only statements that are entailed by the source document."
    \end{enumerate}
}

\subsection{Correlation with Human Judgment}
\itay{is this should be here or in the experiment?}
To evaluate the quality of the evaluation framework, we randomly selected 50 questions along with 402 atomic claims \gabis{where do these claims come from? Gold?}. Three physicians were given instructions on how to perform the task of classifying the logical relationship for each triplet of (question, answer, claim) into one of three NLI categories \itay{[For more information on the instructions and training, please refer to Appendix XX]}. The agreement level among annotators was assessed using Fleiss’ kappa ($\kappa$) and pairwise agreement. For the three human annotators, $\kappa=0.698$, and for the four raters (including our LLM-based evaluation model), the results yielded $\kappa=0.678$. The pairwise agreement among human annotators was found to be $83.2\%$, and with the evaluation model, it was $81.3\%$.
\nadav {should we mention this in the abstract?}\itay{it is written there as "Our findings demonstrate that our evaluation framework performs on par with human medical professionals" - I don't think that we need more numbers}
% resulted in ..., representing medium inter-annotator agreement. 

% For a subset of questions in \kqa{}, 3 physician received an annotation task, were they had to classify the logical relationship between the generated responses of various of LLMs to the medicaly trustful atomic claims. We estimated Fleiss’s Kappa ($\kappa$) to assess the inter-annotator agreement. For 3 human annotators $\kappa=0.698$, and for the 4 raters (including our LLM-based evaluation model) the results were $\kappa=0.678$.  
% Disagreement within experts highlights the challenges of judging the logical relationship the subjectivity of the matter. There are many salient properties of long-form answers, which we discuss next, and deciding how to value each property when coming up with an overall preference is highly subjective (see Appendix Table 8 for several examples)

\input{tabels/evaluation_comparison}

==> sections/08_limitations.tex <==
\label{sec:limitations}
\textbf{Scope of our evaluation method}. 
One limitation is our inability to catch hallucinations that do not explicitly contradict the original claims. As a result, we cannot effectively verify the truthfulness of parts of the generated answers that are not mentioned in the claims. 
Furthermore, we may encounter difficulties in handling high-definition specifications, particularly when dealing with numerical values, as agreeing or contradicting such specifics might prove intricate.
In addition, our evaluation method faces constraints when analyzing statements that are not fully self-contained, limiting its ability to grasp contextual nuances and interconnected ideas.
Lastly, while we have incorporated LLM as an automatic evaluator to reduce time and costs compared to human evaluators, there is still a cost associated with using these sophisticated models for evaluation. Nonetheless, it remains a more cost-effective approach compared to relying solely on human evaluation.



==> sections/09_acknowledgments.tex <==
\label{sec:acknowledgments}
\textbf{Acknowledgments}. 
We would like to thank Noah Smith, Yoav Goldberg, and Jonathan Berant for insightful discussio

==> sections/99_defs.tex <==

% \renewcommand{\draftcomment}[3]{}  % uncomment for submission

\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{multirow}


\definecolor{bottlegreen}{rgb}{0.0,0.42,0.31}
\definecolor{donorred}{RGB}{228.,116.,95.}
\definecolor{reciepientblue}{RGB}{0,152,251}

\newcommand{\draftcomment}[3]{{\textcolor{#3}{[#1]#2}}}
\newcommand{\gabi}[1]{\draftcomment{#1}{\textsc{gabi}}{red}}
\newcommand{\itay}[1]{\draftcomment{#1}{\textsc{Itay}}{blue}}
\newcommand{\naama}[1]{\draftcomment{#1}{\textsc{Naama}}{purple!80}}
\newcommand{\yaara}[1]{\draftcomment{#1}{\textsc{Yaara}}{green}}


\newcommand{\nadav}[1]{\draftcomment{#1}{\textsc{Nadav}}{olive}}
\newcommand{\gabis}[1]{\gabi{#1}}
\newcommand{\gabirep}[2]{\gabi{\sout{#1} #2}}
\newcommand{\gabist}[1]{\gabi{\sout{#1}}}
\newcommand{\itayst}[1]{\itay{\sout{#1}}}
\newcommand{\gabisrep}[2]{\gabirep{#1}{#2}}

% project-specific
\newcommand{\cg}[0]{ChatGPT}
\newcommand{\oai}[0]{OpenAI}
\newcommand{\nsamples}[0]{\gabis{7,777}}
\newcommand{\ntasks}[0]{\gabis{32}}
\newcommand{\bleu}[0]{BLEU}
\newcommand{\ghlink}[0]{github.slab/TODO}
\newcommand{\mh}[0]{Must\textunderscore have }
\newcommand{\nth}[0]{Nice\textunderscore to\textunderscore have}
% \newcommand{\kqa}[0]{MedAsk}
\newcommand{\kqa}[0]{\textsc{CayQA}}
\newcommand{\askk}[0]{AskK}
\newcommand{\ro}[0]{ROUGH}
\newcommand{\bl}[0]{BLEU}

\newcommand{\checked}{\ding{51}}
\newcommand{\crossed}{\ding{55}}

\newcommand{\example}[1]{\emph{``#1''}}
\newcommand{\numofcurated}[0]{201}
\newcommand{\numofraw}[0]{NUM-OF-RAW-QS}
\newcommand{\khealth}[0]{K Health}

==> tabels/app_res.tex <==
\begin{table}[h] 
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{\emph{Comp} $\uparrow$} & \multicolumn{3}{c}{\emph{Hall} $\downarrow$} & \multirow{2}{*}{\# unanswered} \\
\cmidrule(lr){2-7}
& {base} & {unanswered} & {\% change} & {base} & {unanswered} & {\% change} & \\
\midrule
GPT-3.5 & 56.2 & 35.4 & 58.8 & 27.9 & 54.5 & 48.9 & 22 \\
GPT-3.5+PE & 59.8 & 55.0 & 8.7 & 23.5 & 36.4 & 35.4 & 22\\						
GPT-3.5+PE+RAG & 65.5 & 62.2 & 5.3 & 16.1 & 18.2 & 11.7 & 21\\
\midrule
GPT-4 & 57.5 & 53.1 & 8.1 & 23.9 & 23.5 & -1.5 & 17 \\ 	
GPT-4+PE & 67.7 & 66.0 & 2.5 & 25.4 & 23.5 & -7.8 & 17\\ 
GPT-4+PE+RAG & 65.2 & 57.6 & 13.1 & 24.4 & 11.8 & -107.3 & 17\\	
\bottomrule
\end{tabular} 
\caption{}
\label{tab:unans_res}
\end{table}


==> tabels/classic_eval_results.tex <==
\begin{table}[tb!]
\label{tab:classic}
\begin{tabular}{@{}lllll@{}}
\toprule
Model     & ROUGE-L & - & BARTScore &  \\ \midrule
     &         &        &      &  \\
     &         &        &      &  \\
     &         &        &      &  \\
Bard & (0.01167, rank) &        &      &  \\
Bing & 0.02522 &        &      &  \\
Ours & & & & \\
\bottomrule
\end{tabular}
\end{table}

==> tabels/dataset_table.tex <==
\begin{table*}[tb!]
\centering
\begin{tabular}{@{}lllrllr@{}}
\toprule
Dataset & Environment & \begin{tabular}[c]{@{}c@{}}Average of \# Words \\ Q / A \end{tabular} & \begin{tabular}[c]{@{}c@{}}Medical \\ \# Q-A Pairs \end{tabular} & \begin{tabular}[c]{@{}c@{}}\# Atomic \\ \ claims \end{tabular} 
\\ \midrule


\begin{tabular}[l]{@{}l@{}}LiveQA \\\cite{abacha2017overview} \end{tabular} & CHiQA & & 738 &\\ 
\midrule

\begin{tabular}[l]{@{}l@{}}MedicationQA\\\cite{BenAbacha:MEDINFO19} \end{tabular}  & MedlinePlus & & 691 &\\
\midrule

\begin{tabular}[l]{@{}l@{}}MEDIQA-AnS \\\cite{savery2020question}  \end{tabular} &  CHiQA & 13 / 80 &  156   & (*)   \\
\bottomrule

\kqa{}     &  \begin{tabular}[l]{@{}l@{}}patient-physician \\interaction \end{tabular} & 13 / 80 &  47    & 100  \\
\bottomrule
\end{tabular}
\caption{Comparison of \kqa{} to previous benchmarks in the area of consumer-health information-seeking. A \itay{v, x or v} indicates a dataset contains a particular feature, is absent, or is partially represented. Please refer to the text for a more detailed discussion.\yaara{where?}}
\label{tab:datasets}
\end{table*}


==> tabels/evaluation_comparison.tex <==
% \begin{table}[tb!]
% \centering
% \begin{tabular}{@{}lllrllr@{}}
% \toprule
% Model      & Agreement       
% \\ \midrule
% Roberta-mnli \cite{liu2019roberta}     & 0.97  \\ 
% GPT-3.5 (zero-shot)     & 0.97   \\
% GPT-4 (zero-shot)     & 0.97   \\
% GPT-4 (FS \& CoT)      & xx    \\ \midrule   
% Human experts    & xx \\
% \bottomrule
% \end{tabular}
% \caption{\itay{DELETE -- WON'T BE SHOWN AS A TABLE}}
% \label{tab:nli_comparison}
% \end{table}

